Trace Inclusion for One-Counter Nets Revisited

One-Counter nets (OCN) consist of a nondeterministic finite control and a single integer counter that cannot be fully tested for zero. They form a natural subclass of both One-Counter Automata, which allow zero-tests and Petri Nets/VASS, which allow multiple such weak counters. The trace inclusion problem has recently been shown to be undecidable for OCN. In this paper, we contrast the complexity of two natural restrictions which imply decidability. First, we show that trace inclusion between an OCN and a deterministic OCN is NL-complete, even with arbitrary binary-encoded initial counter-values as part of the input. Secondly, we show Ackermannian completeness of for the trace universality problem of nondeterministic OCN. This problem is equivalent to checking trace inclusion between a finite and a OCN-process.

==> app_universality.tex <==
First, due to \cref{lem:macroprops}, we know that in order to analyse traces of
a process $pm$ of $\NN{N}$, we can speak about macrostates of $\NN{N}$.
Observe that if there is a word $w\in\Act^*$ which is not a traces of
$pm$ then it has to start from $\sharp$ letter.
After reading the first letter $\sharp$, the macrostate of the $\NN{N}$
corresponds to the initial configuration of the \incCM.
The main invariant that justifies the contruction is as follows.
Let $f$ and $g$ be corresponding configuration of \incCM\ and a macrostate of $\NN{N},$ respectively;
\begin{enumerate}
\item for any valid move of \incCM\ from $f$ to $f'$ there is a letter $a$ such that it forces a move from $g$ to $g'$
and $f'$ corresponds to $g'$.
\item for any move via letter $a$ from $g$ to $g'$ such that $g'$ does not contain $U$ the universal state there is a 
move of \incCM\ from $f$ to $f'$ such that $f'$ corresponds to $g$. 
\end{enumerate}
Both properties can be easily proven by analysis case by case possible moves and responses for them.

Second important fact is that any word $w$ which does not belong to traces of $\NN{N}$ must have three properties:
\begin{enumerate}
\item any prefix of $w$ can not lead to a macrostate that contains $U$ the universal state,
\item $w$ must contain letter $\$$.
\item if $w$ is of a form $\sharp v \$ v'$ and word $\sharp v \$ $ does not lead to a macrostate that contains $U$ the universal state then $w$ does not belong to traces of $\NN{N}$.
\end{enumerate}

Combining these five facts it is easy to see that any accepting run of \incCM\ can be translated into a word that do not belong to traces of $\NN{N}$ and vice-versa. 
    

 
 
 
 
Namely, for any accepting run $r$ of \incCM\ there is a word $w$ which is not a trace of $\NN{N}.$ The word $w$ starts form $\sharp$ then 
there is a word that corresponds to $r$ and finally symbol $\$$ twice. Observe that rules according to which $\NN{N}$ is build guarantee
that after first $\$$ the macrostate equals $\{\bot\cdots \bot \}$, so second $\$$ goes outside of set of traces.

%\paragraph{only if direction}
%Observe that any word $w$ which does not belong to the set of traces of $\NN{N}$ can not go through a macrostate that contains a process $U$ so it means that the first symbol has to be $\sharp$. Moreover after reading $\sharp$ there is a strict correspondence between
%macrostate of $\NN{N}$ and the initial configuration of \incCM. In addition rules translation guaranties that each move of 
%$\NN{N}$ that does not introduce $U$ into the macrostate can be translated into a move of \incCM\ such that 
%macrostate of $\NN{N}$ after the move corresponds to the configuration of \incCM\ after the move. Now observe that, 
%only words that contain letter $\$$ may do not belong to traces of $\NN{N}$ and that in such case the first $\$$ in $w$ has to appear in the position when 
%macrosatate contains process in final state. From this we conclude that the word which do not belong to traces of $\NN{N}$ has to induce an accepting run of \incCM. 
%\qed
%
%Moreover to each counter we add a decreasing transition labelled with $\sharp$ that leads to universal state. Using it
%Pathfinder can remove counters if all of them are zero and if she is in final state, otherwise she will be punished by going to universal state.
%
%From above one can see that if Pathfinder adds to the word a letter which correspond to an action which is not a  valid action in
%$CA$ then she losses because of universal state. On the other side if she faithfully reaches final configuration she can play $\sharp$ and win. Moreover this is the only way how Pathfinder can win, because$ \Zero$ generates all traces without second $\sharp$.
%
%
%
%  We show how only how to enforce faithful increments, decrements are
%    analogous. Assume line $S_i$ of the $CM$ reads $c_1:= c_1+1; \mathit{goto} S_j$.
%    This means we need to enforce a path
%    $\{S_i:0,C_1:n, \ol{C}_1:l-n,C_2:m,\ol{C}_2:l-m\}$
%    $\WStep{}{*}{}\{S_j:0,C_1:n+1, \ol{C}_1:l-n-1,C_2:m,\ol{C}_2:l-m\}$
%    and punish, i.e., make it unavoidable to mark $U$ in case the counter-value $n=l$
%    already reached the limit $l$.
%
%    The idea is to spawn an obstacle, a new instance of the counting net
%    that allows to count up to $l$ and reach $U$ when it does.
%    At the same time, we spawn a simple ``count down'' state $T$ ignores all
%    actions in $\Act_k$ other than $0$, in which case it decreases.
%    See figure \TODO{}.
%    The crucial aspect is that $T$ can play a ``kill''-action and become universal
%    by a transition $T\step{kill,-1}U$ and no state in the counting gadget
%    has such an action. This means that if pathfinder is able to
%    decrement the dimension $T$ to $0$, it is safe to play the $kill$-action
%    and thereby remove $T$ as well as the complete counting gadget.
%    This can be done precisely if initially, the value of counter $C_1$ was
%    $<l$. Otherwise, if the countdown starts with value $l$, pathfinder has no option
%    other than faithfully simulating the recursive computation of $F_k(1)=l$
%    in the counting net, which inevitably ends with marking the universal state $U$.
%
%    \paragraph{Zero-Tests.}
%    Implementing zero-tests is trivial: all one needs to do to punish
%    unfaithful operations $Z_i$ that announce the condition $C_i==0$
%    is to add transitions $C_i\step{Z_i, -1} U$, that mark $U$
%    with value $C_i\neq\bot$ unless the value of $C_i$ was in fact $0$.


==> definitions/decompositions.tex <==
\begin{definition}[Path Decompositions]\label{def:decompositions}
    Let $\pi\in E^*$ be a path in the product graph. A (loop)
    \emph{decomposition} of $\pi$ is a sequence
    \begin{equation*}
        (\pi_0,L_0,l_0)
        (\pi_1,L_1,l_1)
        \dots
        (\pi_k,L_k,l_k)
        \pi_{k+1}
    \end{equation*}
    in $(E^*\x E^*\x\N)^*E^*$
    such that
    1) $\pi=\pi_0L_0^{l_0}\pi_1L_1^{l_1}\dots\pi_kL_k^{l_k}\pi_{k+1}$,
    2) $L_i$ is a loop for every $0\le i\le k$ and
    3) $\pi_i$ is acyclic for $0\le i \le k+1$.
    %
    A decomposition is called \emph{eager} if
    for any two transitions 
    $t\in \pi_i$ and $t'\in L_i$ with $target(t)=target(t')$,
    we have
    $target(L_i)=target(t)$.
    That is, if a loop $L_i$ shares exactly one node with the
    acyclic path $\pi_i$ it succeeds.
    %
    We see that every path $\pi$ admits exactly one eager decomposition
    $Dec(\pi) = (\pi_0,L_0,l_0)(\pi_1,L_1,l_1)\dots(\pi_k,L_k,l_k)\pi_{k+1}$.
    %which we will call \emph{the} decomposition of $\pi$ in the following.
    Let $Loops(\pi)$ denote the tuple $(L_0,L_1,\dots,L_k)$
    of loops that occur in $Dec(\pi)$.
\end{definition}

%Observe that $Loops(\pi)$ does not only contain information about
%which loops occur in the unique eager decomposition of $\pi$,
%but also about in which order they occur.


==> definitions/ocp.tex <==
\begin{definition}[One-Counter Processes]
    A \emph{one-counter automaton} (OCA) $A=(Q,\Act,\delta,\delta_0)$
    is given by a finite set
    of control-states $Q$, a finite set of action labels $\Act$
    and transition relations $\delta\subseteq Q\x \Act\x\{-1,0,1\}\x Q$
    and $\delta_0\subseteq Q\x \Act\x\{0,1\}\x Q$.
    It induces an infinite-state labelled transition system over
    the stateset
    $Q\x\N$, whose elements will be written as $pm$, as follows.
    $pm\step{a}p'm'$ iff
    \begin{enumerate}
      \item $t=(p,a,d,p')\in\delta$ and $m'=m+d\ge0$ or
      \item $t=(p,a,d,p')\in\delta_0$, $m=0$ and $m'=d$.
    \end{enumerate}
    Abusing notation, we also write $pm\step{t}qn$ if transition $t$ justifies step $pm\step{a}p'm'$
    as above.
    Such an automaton is called a \emph{one-counter net} (OCN) if
    $\delta_0=\emptyset$, i.e., if the automaton 
    cannot test if the counter is equal to $0$.

    A OCA is \emph{complete} if for every pair $(p,a) \in Q\x\Act$ there
    is at least one pair $(d,q)\in\N\x Q$ with $(p,a,d,q)\in\delta\cup\delta_0$.
    It is \emph{deterministic} if for every pair $(p,a) \in Q\x\Act$ there
    is at most one pair $(d,q)\in\N\x Q$ with $(p,a,d,q)\in\delta\cup\delta_0$.
    %
    By \emph{one-counter process} we mean a configuration $pm$ of a OCA.
\end{definition}
    We extend the step relation $\step{}$ to words over $\Act$
    (and $\delta$) inductively in the standard way.
    In the following we will be interested in (deterministic) OCN only
    and will therefore omit $\delta_0=\emptyset$ whenever possible.

\begin{property}[Monotonicity]\label{prop:monotonicity}
    Let $N=(Q,\Act,\delta)$ be a OCN. For all $p\in Q$,
    $a\in\Act$ and $m,l\in\N$ holds that
    If $pm\step{a}p'm'$ then $p(m+l)\step{a}p'(m'+l)$.
\end{property}


==> definitions/traces.tex <==
\begin{definition}[Traces]
  A \emph{labelled transition system} is described by a triple
  $S=(V,\Act,\step{})$ where $V$ is a (possibly infinite) set of
  states, $\Act$ is a finite set of action labels and $\step{}\subseteq V\x
  \Act\x V$ is the labelled transition relation.
  We use the infix notation $s\step{a}s'$ for a transition $(s,a,s')\in\step{}$
  and extend the transition relation to words over $\Act$ in the usual fashion.
  A state $\alpha \in V$ is called a \emph{process}.
  %
  The \emph{traces} of a process $\alpha$ are the elements of the set
  \begin{equation*}
    T(\alpha)=\{w\in\Act^*\ |\ \exists \alpha'\  \alpha\Step{w}{}{}\alpha'\}.
  \end{equation*}
  \Tinc\ is the decision problem that asks if $T(\alpha)\subseteq T(\beta)$
  holds for given processes $\alpha$ and $\beta$.
  \Tuniv\ asks if $\Act^*\subseteq T(\alpha)$ holds for a given
  process
  $\alpha$.
\end{definition}


==> definitions/weights.tex <==
\newcommand{\LO}[1]{\prec_{#1}}
\newcommand{\LOL}{\LO{\mathcal{L}}}
\newcommand{\SOL}{\sigma_{\mathcal{L}}}

\begin{definition}[Weights]
    \label{def:weights}
Let us fix, for every possible finite sequence $\mathcal{L}=(L_0,L_1,\dots,L_k)$
of loops, some linear order $\LOL$ on $\{L_0,L_1,\dots,L_k\}$ that satisfies the following
conditions where
%$L,L'$ are loops with
$i$ and $j$ minimal such that $L=L_i$ and $L'=L_j$.

\begin{enumerate}
    \item\label{cond:PL} If $Type(L)=Type(L')=\TypeUU$ and $S(L)\ge S(L')$ then $L'\LOL L$.
    \item\label{cond:PLE} If $Type(L)=Type(L')=\TypeUU$ and $S(L)=S(L')$ and $i<j$ then $L'\LOL L$.
    \item\label{cond:PR} If $Type(L)=Type(L')=\TypeUU$ and $S(L)<S(L')$ then $L\LOL L'$.
    \item\label{cond:NL}  If $Type(L)=Type(L')=\TypeDD$ and $S(L)<S(L')$ then $L'\LOL L$.
    \item\label{cond:NR}  If $Type(L)=Type(L')=\TypeDD$ and $S(L)>S(L')$ then $L\LOL L'$.
    \item\label{cond:NRE}  If $Type(L)=Type(L')=\TypeDD$ and $S(L)=S(L')$ and $i<j$ then $L\LOL L'$.
\end{enumerate}

Based on $\LOL$ we define the permutation $\SOL:\underline{k}\to\underline{k}$
by $\SOL(i)<\SOL(j)\iff L_i\LOL L_j$.
%We are now ready to define a measure $W$ of paths.
Let $\pi$ be a path with
$Dec(\pi) = (\pi_0,L_0,l_0)(\pi_1,L_1,l_1)\dots(\pi_k,L_k,l_k)\pi_{k+1}$ and let
$\sigma$ be the permutation $\sigma_{Loops(\pi)}$.
We define 
\begin{equation}
  W(\pi)=(l_{\sigma(0)},l_{\sigma(1)},\dots,l_{\sigma(k)}) \in \N^k.
\end{equation}
\end{definition}


==> pictures/pic_univ_gadget.tex <==
  \begin{tikzpicture}[node distance=2.5cm]

      \node[state] (F0) at (0,0)     {$F_0$};
      \node[state, left of=F0] (F1)  {$F_1$};
      \node[state, left of=F1] (F2)  {$F_2$};
      \node[state, left of=F2] (F3)  {$F_3$};
      \node[state, above of=F1] (A)  {$Akk$};
      \node[state, below of=F1] (U)  {$U$};
      
      \draw[->] (A) edge[loop right] node {$1,+$} (A);

      \draw[->] (F0) edge[loop right] node {$1,-$} (F0);
      \draw[->] (F1) edge[loop right] node {$2,-$} (F1);
      \draw[->] (F2) edge[loop right] node {$3,-$} (F2);
      \draw[->] (F3) edge[loop right] node {$4,-$} (F3);
      
      \draw[->] (A) edge[] node[right] {$2$} (F0);
      \draw[->] (A) edge[] node[right] {$3$} (F1);
      \draw[->] (A) edge[] node[right] {$4$} (F2);
      
      
      \draw[->] (F0) edge[] node[right] {$2,3,4$} (U);
      \draw[->] (F1) edge[] node[right] {$3,4$} (U);
      \draw[->] (F2) edge[] node[right] {$4$} (U);
  \end{tikzpicture}


==> proofs/form.sketch.tex <==
%\begin{proofof}{Theorem \ref{thm:form}}
%\begin{proof}
    %We show that we can sufficiently increase a 
    We stepwise approximate
    %We show that we can 
    polynomial $\fbound$
    large enough
    such that whenever $T(pm)\not\subseteq T(qn)$ but no witness
    shorter than $\fbound$ exists, as well as none of forms 1) or 2),
    then there must be a witness of form 3).
    
    Initially, let $c:=F_0$, the number of different loop effects.
    Assume $T(pm)\not\subseteq T(qn)$ and consider a reduced witness, % $\pi$,
    that is minimal in length.
    %no shorter witness is reduced.
    %Recall that this also means that $\pi$ is sane: it is of form
    %described in \cref{eq:form:sane}.
    We can decompose any such witness $\pi$ as in \cref{eq:form:sane} %$\pi$ as
    %\begin{equation}
    %    \label{eq:form:sketch}
    %    \pi=\pi_0L_0^{l_0}\pi_{1}L_{1}^{l_1}\dots\pi_kL_k^{l_k}\pi_{k+1}
    %\end{equation}
    where $r$ and the length of all $\pi_i$ is at most $|V|$.
    By monotonicity (\cref{lem:witness-monotonicity})
    and minimality, %and because $\pi$ is of minimal length
    %among the reduced witnesses,
    we see that none of the loops $L_i$ is of type $\TypeDU$.
    %TODO: necessary?
    %In the following we simply write $L_i$ for the $i^{\text{th}}$ loop occurring
    %in the decomposition \eqref{eq:form:dec} of $\pi$.
    Moreover, because $\pi$ is not of form 1), % we can safely assume that $\pi$
    it contains
    only loops of types $\TypeUU$ and $\TypeDD$.
%
    %We now relax the bound on the 
    Relaxing the bound on the
    length of intermediate paths $\pi_i$ between loops
    allows us to ``unroll'' some subobtimal loops
    that, by \cref{lem:bounds}, are iterated only a few times.
    This way, by stepwise allowing longer
    (polynomially bounded) subpaths,
    and excluding more ``bad'' forms,
    we are eventually able to conclude that
    %the current bound is
    %sufficient to ensure thaat
    any
    witness longer than the current approximated bound $\fbound$
    which is not of form 1) or 2) must have form 3).
    \qed
%\end{proofof}
%\end{proof}


==> testfile.tex <==
aaaaaa


==> udraft.tex <==
\begin{definition}

By incrementing counter automaton we define counter automaton in which counters can spontaneously increment without performing any transitions. Such increments we call incrementing errors.

\end{definition}


\todo{control automaton}


By a configuration we mean state and counters valuation.

\begin{definition}

Reachability

\end{definition}


\begin{theorem}[reference]

The reachability problem for incrementing one counter automaton is not

primitive recursive hard.

\end{theorem}


\begin{remark}

Even if we restrict initial and final configurations to configurations with all counters empty. In the following we assume that initial and final configurations are of this form.

\end{remark}


\begin{remark}

Let $r$ be a run of an incrementing counter automaton from initial to final configuration. Then there exists a run $r_1$ form initial to final configuration in which all incrementing error increments counter from value $0$ to value $1$ and are followed by the

decrement operation on the same counter.

\end{remark}

\begin{proof}

We postpone all incrementing errors in $r$ as much as possible.

\end{proof}


In the following we restrict only to simple runs that goes from initial to final configuration.


Now for a given incrementing counter automaton $CA$ we will define one counter net $N$ such that traces of $N$ are not universal

iff there is a run of $CA$.


The basic idea is to add to every transition of $CA$ a unique label and to build $N$ in such a way that a run $r$ induces a word $W$ such that $w\sharp$ where $\sharp$ is a special letter

is a witness for the non universality of $N$.


By constellation of a net after reading a word $w$ we mean a set of configurations in which $N$ can be after reading a word $w$.

To talk about nonuniversality we define

a following one player game which is played in rounds.

Spoiler (the name of the player) builds a word in each round adding one letter on it's end. She wins if the obtained word is witness for non universality of traces of the net $N$ and looses if one can easily verify that current word $w$ can not be a prefix of a witness.

By easily verify we mean that in in the constellation after reading $w$ there is an universal configuration that can loops on every letter, or

if the constellation after reading $w$ is bigger than a constellation after reading $w_1$ some prefix of $w$.


One can see that Spoiler wins the game iff traces are not universal for the net $N$.


\paragraph{Construction}


The net $N$ will consist from five parts which are responsible for different tasks. They are initial state, universal state, incrementing, finite automaton, counters end error state. The initial state is responsible to set up the proper initial constellation. Universal state

is used by automaton to punish spoiler if he tries to make a move that do not simulate a valid move of

$CA$. Finite automaton $FA$ has the same set of states and transitions as control automaton of $CA$ all those transitions do not change

values of the counter. In addition for every state $s$ in $FA$ and for every label $a$ in $CA$ if there is no outgoing $a$ transition

we add one which lead to universal state. This allow to punish Spoiler if she tires to perform an action that is not available in the state $s$ in $CA$. Finally to every state except of final state we add a transition to universal state labelled with $\sharp$. This allow Spoiler to play

$\sharp$ only if she reaches a constellation that contains a configuration with final state. The \emph{initial constellation} contains only one

configuration with state from $(FA)$ and it is easy to see that after reading any word $w$ constellation contains no more than

$1$ configuration with state form $(FA)$.


Counters is the set of $k$ states where $k$ is the number of counter in $CA$.

In the initial constellation there is exactly one configuration for each counter with counter-value equal to $0$. Each of those

configuration is responsible to simulate corresponding counter in $CA$. Every move in $CA$ can do one on the following with the counter: increment it, decrement it, do nothing with it, check if its value equals $0$. We have to describe what is going with the

counter in each of those cases.

\begin{enumerate}

\item If the transition labelled with $a$ increases the counter $c$ then in $N$ the will be a transition from $c$ to $c$ labelled with $a$ which increments the counter.

\item If the transition labelled with $a$ do nothing the counter $c$ then in $N$ the will be a transition from $c$ to $c$ labelled with $a$ which do nothing the counter.

\item If the transition labelled with $a$ test equality of the counter $c$ to $0$ then in $N$ the will be a transition from $c$ to $c$ labelled with $a$ which do not change the value the counter and a transition labelled with $a$ from $c$ to universal state that decreases the counter. Observe that if $a$ was chosen by Spoiler and the counter-value is grater than $0$ then she losses because

game reaches universal state, so Spoiler is punished if she tries to cheat on zero testing transition.

\item If the transition labelled with $a$ decrements the counter $c$ then in $N$ the will be a transition from $c$ to $c$ labelled with $a$ decrements the counter. However observe that this do not suffice because if the value of the counter was $0$ then this move

remove counter from the constellation. In $CA$ such decreasing transition is performed with incrementing error, so we have to do the same here. That is why we add a transition labelled with $a$ which do not change the counter-value from the error state to the $c.$

The configuration that contains error state have counter-value equal to $0$ thus, after decreasing move we are sure that there will be a counter $c$ with value at least $0$. The suspicious could be fact that such a transition will produce a configuration even if the counter-value $c$ is grater than $0$ so this leads to several configurations with state $c$. This is not a problem due to observation that

the .......... \todo{bigger}

\end{enumerate}

Moreover to each counter we add a decreasing transition labelled with $\sharp$ that leads to universal state. Using it

Spoiler can remove counters if all of them are zero and she is in final state, otherwise she will be punished by going to universal state.



Error state loops without changing the value of the counter on every label except of $\sharp$. The initial constellation contains

a configuration with error state and counter-value equals $0$.

From above one can see that if Spoiler add to the word letter which correspond to action which is not valid action in

$CA$ then he losses because of universal state. On the other side if she faithfully reaches final configuration she can play $\sharp$ and win. Moreover this is the only way how Spoiler can win, for example due to error state which contains all traces without $\sharp$.




==> univ-bad-witnesses.tex <==
%%%
% I AM NOT USED IN THE PAPER AND JUST HERE FOR THE THESIS
%%%


\paragraph{Counting Gadgets.}
For fixed $k\in\N$ we consider the net
over the action alphabet $\Act=\{0,1,\dots,k\}\cup\{e\}$
that contains, apart from a universal state $U$,
\begin{enumerate}
  %\item a universal state $U$,
  \item states $F_i$ for $0\le i\le k$,
      each of which
      has a $i$-labelled counter decreasing self-loop
      and is an obstacle for $e$ and all larger actions $j>i$.
      %and a $e$-labelled step to $U$.
  \item An accumulator-state $A$ with a counter-increasing self-loop labelled by $0$
      and $(i+1)$-labelled steps to $F_i$ for all $i<k$.
\end{enumerate}
%Moreover,
%for every $i<k$, the state $F_i$ allows steps
%$F_i\step{j,0}U \in\delta$ for labels $j>i$.
See \cref{fig:counting_gadget} for this net for $k=3$.
We observe the following important property of these nets.

\begin{figure}[h]
\begin{center}
    \includegraphics[scale=0.7]{pictures/pic_univ_gadget.pdf}
\end{center}
\caption{The counting net for $k=0$. The effect of transitions on the counter
is $0$ if not explicitly stated. The self-loop at state $U$ indicates
steps $U\step{a,0}U$ for all actions $a$.\TODO}
\label{fig:counting_gadget}
\end{figure}

\begin{lemma}\label{lem:counting_gadgets}
    The macrostate $\{A=m, F_k=n\}$
    is not universal, but any witness
    ends in a $e$-step from macrostate $\{A=l\}$
    for some $l\ge F_k^n(m)$.
\end{lemma}
Intuitively, in order to show non-universality, a pathfinder must
play the ``end''-action $e$ eventually. For this,
all occurrences
%play the ``end''-action $e$ but avoid macrostates with $M(U)\neq\bot$.
%This is only possible by removing all occurrences 
of obstacles $F_i$ must first be removed
by faithfully recurring and thus counting up to at least $F_k^m(n)$.


